Feature Selection for Linear SVM with Provable Guarantees

We give two provably accurate feature-selection techniques for the linear SVM. The algorithms run in deterministic and randomized time respectively. Our algorithms can be used in an unsupervised or supervised setting. The supervised approach is based on sampling features from support vectors. We prove that the margin in the feature space is preserved to within $\epsilon$-relative error of the margin in the full feature space in the worst-case. In the unsupervised setting, we also provide worst-case guarantees of the radius of the minimum enclosing ball, thereby ensuring comparable generalization as in the full feature space and resolving an open problem posed in Dasgupta et al. We present extensive experiments on real-world datasets to support our theory and to demonstrate that our method is competitive and often better than prior state-of-the-art, for which there are no known provable guarantees.

==> bss_algo.tex <==
\subsection{Our main tool: Spectral Sparsification of an Orthogonal Matrix}
\label{sec:main_tool}
We describe the main tool from 
linear algebra that we will use to do feature selection: a 
spectral sparsification algorithm for an orthogonal matrix
 (\textbf{BSS}\footnote{The name BSS comes from the authors of the
algorithm Batson, Spielman and Srivastava of \cite{BSS09}.} for short).
The details of the algorithm, which we defer to the
supplementary material, are not important for our
presentation -- the sparsification property of the algorithm is 
all we will need to prove our results.
Consider an \math{\ell\times d} matrix (\math{\ell} rows in 
\math{d} dimensions),
$\matV^T = \left[ \v_1, \v_2,....,\v_d \right]$, 
with $\v_i \in \mathbb{R}^\ell$. The BSS algorithm samples \math{r} columns in 
$O\left(rd\ell^2 \right)$ time to construct a sparsifier \math{\matR}
for which 
\math{\matV^T\matV\approx\matV^T\matR\matR^T\matV}.
\begin{lemma}[\textbf{BSS}, \cite{BSS09}] \label{lem:ssp}
Let $\matV \in \mathbb{R}^{d \times \ell}$ satisfy 
$\matV^T\matV = \matI_\ell$ and $r>\ell$. 
There is a deterministic algorithm running in 
\math{O\left(rd\ell^2 \right)} time to construct
 sampling and rescaling matrices $\matS \in \mathbb{R}^{d \times r}$ 
and $\matD \in \mathbb{R}^{r \times r}$ such that for $\matR= \matS\matD$, 
\mand{\norm{ \matV^T\matV - \matV^T\matR\matR^T\matV}_2 \leq 3\sqrt{\ell/r}}
\end{lemma}
\begin{proof}(sketch)
BSS \cite{BSS09} proves
\math{\sigma_i^2(\matV^T\matR)=(1\pm O(\sqrt{\ell/r}))^2}. 
The result follows because
\math{\sigma_i(\matV^T\matV - \matV^T\matR\matR^T\matV)
=
\sigma_i(\matI - \matV^T\matR\matR^T\matV)
=1-\sigma_i^2(\matV^T\matR)}.
\end{proof}

%%
%%\input{sssp}


